Separating Automatic Relations

We study the separability problem for automatic relations (i.e., relations on finite words definable by synchronous automata) in terms of recognizable relations (i.e., finite unions of products of regular languages). This problem takes as input two automatic relations $R$ and $R'$, and asks if there exists a recognizable relation $S$ that contains $R$ and does not intersect $R'$. We show this problem to be undecidable when the number of products allowed in the recognizable relation is fixed. In particular, checking if there exists a recognizable relation $S$ with at most $k$ products of regular languages that separates $R$ from $R'$ is undecidable, for each fixed $k \geq 2$. Our proofs reveal tight connections, of independent interest, between the separability problem and the finite coloring problem for automatic graphs, where colors are regular languages.

==> Makefile <==
TEXFILE = main.tex
KLFILE = header/kl-knowledges.tex
DIAGNOSEFILE = main.diagnose
ZIPFILE = aut-rec-separability.zip

.PHONY: all kl clean Clean init zip

all:
	latexmk -pdf -use-make -synctex=1 -interaction=nonstopmode -file-line-error $(TEXFILE) -silent

kl:
	knowledge cluster -k $(KLFILE) -d $(DIAGNOSEFILE)

clean: # Clean all nonessential files, except dvi, pdf and ps files
	latexmk -c -silent
	rm -f $(DIAGNOSEFILE) *.kaux $(ZIPFILE)

Clean: # Clean all nonessential files 
	latexmk -C -silent
	rm -f $(DIAGNOSEFILE) *.kaux $(ZIPFILE)

zip:
	zip -r $(ZIPFILE) . -x .git\* .gitignore .vscode\* Reg2Rec\*
